A Concept for Reconstructing Stucco Statues from historic Sketches using synthetic Data only

In medieval times, stuccoworkers used a red color, called sinopia, to first create a sketch of the to-be-made statue on the wall. Today, many of these statues are destroyed, but using the original drawings, deriving from the red color also called sinopia, we can reconstruct how the final statue might have looked.We propose a fully-automated approach to reconstruct a point cloud and show preliminary results by generating a color-image, a depth-map, as well as surface normals requiring only a single sketch, and without requiring a collection of other, similar samples. Our proposed solution allows real-time reconstruction on-site, for instance, within an exhibition, or to generate a useful starting point for an expert, trying to manually reconstruct the statue, all while using only synthetic data for training.

==> paper-prob-old.tex <==
\begin{document}

% ---------------------------------------------------------------------
% EG author guidelines plus sample file for EG publication using LaTeX2e input
% D.Fellner, v2.03, Dec 14, 2018


\title[EG \LaTeX\ Author Guidelines]%
      {Single View Geometry Estimation using historic Sketches of Statues}

% for anonymous conference submission please enter your SUBMISSION ID
% instead of the author's name (and leave the affiliation blank) !!
% for final version: please provide your *own* ORCID in the brackets following \orcid; see https://orcid.org/ for more details.
\author[T. Pöllabauer \& J. Kühn]
{\parbox{\textwidth}{\centering T. Pöllabauer$^{1}$\orcid{0000-0001-7756-0901}
        and J. Kühn$^{1}$\orcid{0000-0001-5923-423X} 
        }
        \\
% For Computer Graphics Forum: Please use the abbreviation of your first name.
{\parbox{\textwidth}{\centering $^1$TU Darmstadt \& Fraunhofer IGD, Germany
       }
}
}
% ------------------------------------------------------------------------

% if the Editors-in-Chief have given you the data, you may uncomment
% the following five lines and insert it here
%
% \volume{36}   % the volume in which the issue will be published;
% \issue{1}     % the issue number of the publication
% \pStartPage{1}      % set starting page


%-------------------------------------------------------------------------


\teaser{
 \includegraphics[width=\linewidth]{sinopien.png}
 \centering
  \caption{Reconstructed Point Clouds}
\label{fig:teaser}
}

\maketitle
%-------------------------------------------------------------------------
\begin{abstract}
   We propose a automated method to estimate the 3D geometry of medieval statues, based on sketches from the period (sinopia). We deal with two major problems: First the low data quality (as can be seen in the samples in figure 2) and second the low amount of available data (in our case only 6 samples). We address both problems with a learning based approach by first applying image to image translation techniques before feeding the data to an encoder-decoder architecture trained on a multitude of other statues with 3D geometry available. The result is an automated approach generating 3D point clouds given a single sinopia.
%-------------------------------------------------------------------------
%  ACM CCS 1998
%  (see https://www.acm.org/publications/computing-classification-system/1998)
% \begin{classification} % according to https://www.acm.org/publications/computing-classification-system/1998
% \CCScat{Computer Graphics}{I.3.3}{Picture/Image Generation}{Line and curve generation}
% \end{classification}
%-------------------------------------------------------------------------
%  ACM CCS 2012
   (see https://www.acm.org/publications/class-2012)
%The tool at \url{http://dl.acm.org/ccs.cfm} can be used to generate
% CCS codes.
%Example:
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10010147.10010371.10010352.10010381</concept_id>
<concept_desc>Computing methodologies~Collision detection</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10010583.10010588.10010559</concept_id>
<concept_desc>Hardware~Sensors and actuators</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10010583.10010584.10010587</concept_id>
<concept_desc>Hardware~PCB design and layout</concept_desc>
<concept_significance>100</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[300]{Computing methodologies~Collision detection}
\ccsdesc[300]{Hardware~Sensors and actuators}
\ccsdesc[100]{Hardware~PCB design and layout}


\printccsdesc   
\end{abstract}  
%-------------------------------------------------------------------------
\section{Introduction}

We are given photographs of medieval drawings on stone walls used by a stonemason to sketch the statues he was about to place on these walls. These statues have been destroyed. Now their geometry should be reconstructed using the sketches. 

\begin{figure}[htb]
  \centering
  % the following command controls the width of the embedded PS file
  % (relative to the width of the current column)
  \includegraphics[width=.8\linewidth]{sinopien.png}
  % replacing the above command with the one below will explicitly set
  % the bounding box of the PS figure to the rectangle (xl,yl),(xh,yh).
  % It will also prevent LaTeX from reading the PS file to determine
  % the bounding box (i.e., it will speed up the compilation process)
  % \includegraphics[width=.95\linewidth, bb=39 696 126 756]{sampleFig}
  %
  %
  \caption{\label{fig:firstExample}
           Two samples out of six available for our use case.}
\end{figure}

\section{Related Work}

Reconstructing 3D information from an image is a long withstanding problem in the computer vision community. It is an inherently ill posed problem since the imaging process by design forfeits knowledge about the depicted scene. \\
One way of dealing with this loss of information is the use of multiple images to reconstruct the 3D information. The availability of additional view points reintroduces much of the lost information about the scene. \\
However, the need for multiple images of a single scene greatly reduces the applicability in real world scenarios by requiring either a multi-camera setup or a static scene, photographed from various view points. \\
This constraint led to interest in solving the reconstruction problem via a single view / single image only. Solving the problem with only one view requires the introduction of additional information, for instance knowledge about objects depicted in the scene. \\
Another possible solution, which proved very successful recently is the use of machine learning and especially deep neural networks. These machine learning algorithms can be trained with a wide variety of scenes with available ground truth data and thereby acquire some general scene understanding or, in other words, a useful prior on the basic construction of scenes and their projection on a 2-dimensional image plane. \\
These approaches often lead to impressive results given the ill posed problem, but usually require real world photographs or other realistic imagery, such as renderings. \\
There is a much smaller body of work dealing with geometry estimation based on hand-drawn sketches of various degrees of complexity. These approaches might use segmentation \cite{sketch_figures} and/or estimate depth and normals before fusing the results to different kind of 3D geometry representations.\\
Some works, especially does relying on differentiable rendering, do not require anything but geometric understanding of the imaging process. In our data limited scenario, however, we favor approaches that allow to learn a prior on other, similar, available data. One such often-utilized approach is the use of encoder-decoder architectures.\\
Encoder-decoder architectures break down an input image (usually using a convolutional neural network) into a, compared ot the original image, small vector representation. This vector space is called the latent space. A second network, the decoder gets vectors sampled from this latent space and has to reconstruct the encoded image. 


%-------------------------------------------------------------------------
\section{3D Point Cloud Estimation from Sinopia}

Our proposed solution takes a single frontal photograph of sinopia, painted on the wall. We first use image to image translation to convert this image to more conventional style, similar to a pencil drawing. Next we feed the converted image to an encoder-decoder network, pre-trained on a dataset of statues with geometry information available. We adopt a previous work, namely \city{encoderTemplate} and modify the process for our very different data. We only feed our intermediary sketch representation and reshape the network accordingly. Most importantly we extend the criterion by introduction a reconstruction task, requiring the encoder-decoder network to also reconstruct a monochromatic image of the statue, depicted in the input sketch. This stabilizes training, while also introducing additional queues to the network without requiring additional inputs at inference time. 

\subsection{Data Generation}
Since we have only six images of our target sketches while wanting to use a data driven approach, we have to come up with a source of high quality data.

\subsection{Image to Image Translation}
Only using the gradients of our renderings (or other conventional edge filtering techniques, such as canny edge detection, laplacian, or mixture of gaussians) does not suffice to make them similar to our sinopia images. The remaining domain gap suffices to make our estimation algorithms work well on our training data, but not on our real world images. \\
Therefore we looked into image to image translation and style transfer techniques popularized by works such as \cite{styletransfer_intro_paper}\cite{adain}\cite{stylegan}\cite{cyclegan}\cite{pix2pixhd}. We decided to use the work of \cite{sketchTranslation}. 

\subsection{Encoder Decoder Network}
To make up for our low data quality we need a powerful prior to compensate for the low signal to noise ratio. Among the vast body of work utilising such architectures we decided to base our work on \city{encoderTemplate}. \\
They use an encoder network to extract a powerful representation of a single input image depicting the target object. Next they use the decoder to generate additional views of the same object i.e. they require the network to predict how the object would look like from other perspectives. Using canonical coordinates the point cloud is fused by transforming the geometry from these synthesized views. Finally they use what they call a pseudo-renderer to produce depth images used for optimization. Since this is a 2D projection, this step does not involve any learnable parameters.\\
We modify their approach to suit our needs. 

\textbf{Architectural details}. We modify the original network to process far larger images (640x640), as well as to improve its expressiveness to compensate for the low information input images. \\

\textbf{Training details}. Unlike the original work we do not train in stages. Instead of first pre-training on a limited number of fixed perspectives (the eight corners of a cube) we directly sample poses uniformly on a sphere surounding the target object. We then require the network to transform the object into the target pose. To initialize the network, we use an added reconstruction loss and show 60000 samples while exclusively requiring the network to reconstruct a grayscale version of the rendering, originally used to create the input sketch. After this warm up phase we scale down the reconstruction loss and add the depth estimation and mask criteria. Our image size is set to 640x640 and we reduce the upsampling during the pooling operation from five- to two-times. We also reduce the learning rate to a tenth of the reported number in the original paper, to 1e-5. Instead of generating N views per object per batch, we only generate one. We use 22 statues for training and 2 additional for validation. Our batch size is set to 12. \\

\section{Results}

Our network has to generalize to unseen objects in order to solve the proposed problem. Therefore we only test on unseen objects. Next we apply our technique not only to renderings, but our historic sinopia.  

\subsection{Unseen Test Objects}
First we present qualitative results on renderings from our unseen objects.\\

We also compare the results on a test set, comprising of 7 additional, unseen objects.

\subsection{Sinopia}
Finally we test our model on the six frontal views of our sinopia.\\

We also have models created by a 3D artist. A direct quantitative comparison i.e. via volume would not be useful, since the low expressiveness of the data required the artist to fill in a lot of detail.

\section{Conclusion}

We demonstrated the automated reconstruction of point clouds based on only six medieval sinopia and without requiring any additional sinopia from that or any other time period. We produce all our data via rendering, process the renderings to make them less distinguishable from our target data and then train an encoder-decoder architecture to produce our 3D data, a plausible rendering of the statue geometry. The resulting point cloud can be converted to a mesh or other data representation. 

%-------------------------------------------------------------------------
\subsection{References}

List all bibliographical references in 9-point Times, single-spaced, at the
end of your paper in alphabetical order. When referenced in the text, enclose
the citation index in square brackets, for example~\cite{Lous90}. Where
appropriate, include the name(s) of editors of referenced books.

For your references please use the following algorithm:
\begin{itemize} 
\item \textbf{one} author: first 3 chars plus year -- 
      e.g.\ \cite{Lous90}
\item \textbf{two}, \textbf{three} or \textbf{four} authors: first char
      of each family name plus year --  e.g.\ \cite{Fellner-Helmberg93} 
      or \cite{Kobbelt97-USHDR} or \cite{Lafortune97-NARF}
\item \textbf{more than 4} authors: first char of family name from 
      first 3 authors followed by a '*' followed by the year -- 
      e.g.\ \cite{Buhmann:1998:DCQ} or \cite{FolDamFeiHug.etal93} 
\end{itemize}

For BibTeX users a style file \ \texttt{eg-alpha.bst} and 
\texttt{eg-alpha-doi.bst} \ is available which uses the above algorithm.

For Biber users a style file \ \texttt{EG.bbx} \ is available which uses the above algorithm.
%  Store EG.bbx in the LaTeX distribution, for TeXLive in Windows: C:\texlive\2018\texmf-dist\tex\latex\biblatex\bbx  
%  and update filename database.
%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.

%%%
%%% Figure 1
%%%
\begin{figure}[htb]
  \centering
  % the following command controls the width of the embedded PS file
  % (relative to the width of the current column)
  \includegraphics[width=.8\linewidth]{sampleFig}
  % replacing the above command with the one below will explicitly set
  % the bounding box of the PS figure to the rectangle (xl,yl),(xh,yh).
  % It will also prevent LaTeX from reading the PS file to determine
  % the bounding box (i.e., it will speed up the compilation process)
  % \includegraphics[width=.95\linewidth, bb=39 696 126 756]{sampleFig}
  %
  \parbox[t]{.9\columnwidth}{\relax
           For all figures please keep in mind that you \textbf{must not}
           use images with transparent background! 
           }
  %
  \caption{\label{fig:firstExample}
           Here is a sample figure.}
\end{figure}

If your paper includes images, it is very important that they are of
sufficient resolution to be faithfully reproduced.

To determine the optimum size (width and height) of an image, measure
the image's size as it appears in your document (in millimeters), and
then multiply those two values by 12. The resulting values are the
optimum $x$ and $y$ resolution, in pixels, of the image. Image quality
will suffer if these guidelines are not followed.

Example 1: 
%
An image measures 50\,mm by 75\,mm when placed in a document. This
image should have a resolution of no less than 600 pixels by 900
pixels in order to be reproduced faithfully.

Example 2: 
%
Capturing a screenshot of your entire $1024 \times 768$ pixel display
monitor may be useful in illustrating a concept from your research. In
order to be reproduced faithfully, that $1024 \times 768$ image should
be no larger than 85 mm by 64 mm (approximately) when placed in your
document.


%-------------------------------------------------------------------------
\subsection{Color}

\textbf{Please observe:} as of 2003 publications in the proceedings of the
Eurographics Conference can use color images throughout the paper. No
separate color tables are necessary.

However, workshop proceedings might have different agreements! 
Figure~\ref{fig:ex3} is an example for creating color plates.

%------------------------------------------------------------------------
\subsection{Embedding of Hyperlinks / Typesetting of URLs}

Due to the use of the package \texttt{hyperref} the original behavior
of the command $\backslash$\texttt{url} from the package \texttt{url}
is not available. To circumvent this problem we either recommend to
use the command $\backslash$\texttt{httpAddr} from the 
included package \texttt{egweblnk} (see below) or to replace the
command $\backslash$\texttt{url} by the command $\backslash$\texttt{webLink} 
-- e.g. in cases where $\backslash$\texttt{url} has been used
widely in BibTeX-References. In the latter case we suggest to run
BibTeX as usual and then replace all occurences of $\backslash$\texttt{url}  by
$\backslash$\texttt{webLink}

\noindent
The provided commands for hyperlinks, in a nutshell, are:

\begin{description} \itemsep 1ex
\item [\webLinkFont $\backslash$httpAddr \{URL without leading 'http:'\}]
      \mbox{}\\
      e.g. \  \httpAddr{//diglib.eg.org/handle/10.2312/306}

\item [\webLinkFont $\backslash$httpsAddr \{URL without leading 'https:'\}]
      \mbox{}\\
      e.g. \  \httpsAddr{//diglib.eg.org/handle/10.2312/306}      

\item[\webLinkFont $\backslash$ftpAddr \{URL without leading 'ftp:'\}]
      \mbox{}\\
      e.g. \  \ftpAddr{//www.eg.org/EG/DL/ftpupload}   %

\item[\webLinkFont $\backslash$URL \{url\}]
      \mbox{}\\
      e.g. \  \URL{http://diglib.eg.org/handle/10.2312/306}

\item[\webLinkFont $\backslash$MailTo \{Email addr\}]
      \mbox{}\\
      e.g. \  \MailTo{publishing@eg.org}

\item[\webLinkFont $\backslash$MailToNA \{emailName\}\{@emailSiteAddress\}]
      \mbox{}\\
      e.g. \  \MailToNA{publishing}{@eg.org}

\item[\webLinkFont $\backslash$webLink\{URL without hyperlink creation\}]
      \mbox{}\\
      e.g. \  \webLink{http://www.eg.org/some_arbitrary_long/but_useless/URL}

\end{description}


%------------------------------------------------------------------------
\subsection{PDF Generation}

Your final paper should be delivered as a PDF document with all typefaces
embedded. \LaTeX{} users should use \texttt{dvips} and \texttt{ps2pdf} to
create this PDF document. Adobe Acrobat Distiller may be used in place of
\texttt{ps2pdf}.

Adobe PDFWriter is \emph{not} acceptable for use. Documents created with
PDFWriter will be returned to the author for revision. \texttt{pdftex} and
\texttt{pdflatex} (and its variants) can be used only if the author can
make certain that all typefaces are embedded and images are not downsampled
or subsampled during the PDF creation process.

Users with no access to these PDF creation tools should make available a
PostScript file and we will make a PDF document from it.


The PDF file \emph{must not} be change protected.

%------------------------------------------------------------------------
\subsubsection*{Configuration Notes: dvips / ps2pdf / etc.}

\noindent
\texttt{dvips} should be invoked with the \texttt{-Ppdf} and \texttt{-G0}
flags in order to use Type 1 PostScript typefaces:

\begin{verbatim}
    dvips -t a4 -Ppdf -G0 -o my.ps my.dvi
\end{verbatim}


\noindent
If you are using version 7.x of GhostScript, please use the following method of invoking \texttt{ps2pdf}, in
order to embed all typefaces and ensure that images are not downsampled or subsampled in the PDF
creation process:

\begin{verbatim}
  ps2pdf -dMaxSubsetPct=100 \
         -dCompatibilityLevel=1.3 \
         -dSubsetFonts=true \
         -dEmbedAllFonts=true \
         -dAutoFilterColorImages=false \
         -dAutoFilterGrayImages=false \
         -dColorImageFilter=/FlateEncode \
         -dGrayImageFilter=/FlateEncode \
         -dMonoImageFilter=/FlateEncode \
         mypaper.ps mypaper.pdf
\end{verbatim}


If you are using version 8.x of GhostScript, please use this method in place of the example above:
\begin{verbatim}
  ps2pdf -dPDFSETTINGS=/prepress \
         -dCompatibilityLevel=1.3 \
         -dAutoFilterColorImages=false \
         -dAutoFilterGrayImages=false \
         -dColorImageFilter=/FlateEncode \
         -dGrayImageFilter=/FlateEncode \
         -dMonoImageFilter=/FlateEncode \
         -dDownsampleColorImages=false \
         -dDownsampleGrayImages=false \
         mypaper.ps mypaper.pdf
\end{verbatim}

%------------------------------------------------------------------------
\subsubsection*{Configuration Notes: pdftex / pdflatex / etc.}

\noindent
Configuration of these tools to embed all typefaces can be accomplished by editing the \texttt{updmap.cfg} file
to enable inclusion of the standard (or base) 14 typefaces.

Linux users can run the \texttt{updmap} script to do this:
\begin{verbatim}
updmap --setoption pdftexDownloadBase14 true
\end{verbatim}

Windows users should edit the \texttt{updmap.cfg} files found in their TeX installation directories (one or both
of the following may be present):
\begin{verbatim}
  INSTALLDIR\texmf\web2c\updmap.cfg
  INSTALLDIR\localtexmf\miktex\config\updmap.cfg
\end{verbatim}

Ensure the value for \texttt{pdftexDownloadBase14} is "true," and then follow the instructions found here:
\httpAddr{//docs.miktex.org/manual/} to update your MikTeX installation.

%------------------------------------------------------------------------
\subsubsection*{Configuration Notes: Acrobat Distiller}

We recommend to use a Distiller job options file that embeds
all typefaces and does not downsample or subsample images when creating the PDF document.
%------------------------------------------------------------------------
\subsection{Exclusive License Form}

You must include your signed Eurographics Exclusive License Form 
when you submit your finished paper. We MUST have this form before
your paper can be published in the proceedings.

%-------------------------------------------------------------------------
\subsection{Conclusions}

Please direct any questions to the production editor in charge of
these proceedings.

%-------------------------------------------------------------------------
% bibtex
\bibliographystyle{eg-alpha-doi} 
\bibliography{egbibsample}       

% biblatex with biber
% \printbibliography                

%-------------------------------------------------------------------------
\newpage


\begin{figure*}[tbp]
  \centering
  \mbox{} \hfill
  % the following command controls the width of the embedded PS file
  % (relative to the width of the current column)
  \includegraphics[width=.3\linewidth]{sampleFig}
  % replacing the above command with the one below will explicitly set
  % the bounding box of the PS figure to the rectangle (xl,yl),(xh,yh).
  % It will also prevent LaTeX from reading the PS file to determine
  % the bounding box (i.e., it will speed up the compilation process)
  % \includegraphics[width=.3\linewidth, bb=39 696 126 756]{sampleFig}
  \hfill
  \includegraphics[width=.3\linewidth]{sampleFig}
  \hfill \mbox{}
  \caption{\label{fig:ex3}%
           For publications with color tables (i.e., publications not offering
           color throughout the paper) please \textbf{observe}: 
           for the printed version -- and ONLY for the printed
           version -- color figures have to be placed in the last page.
           \newline
           For the electronic version, which will be converted to PDF before
           making it available electronically, the color images should be
           embedded within the document. Optionally, other multimedia
           material may be attached to the electronic version. }
\end{figure*}

\end{document}

